Neural Topographic Factor Analysis for fMRI Data

Neuroimaging studies produce gigabytes of spatio-temporal data for a small number of participants and stimuli. Rarely do researchers attempt to model and examine how individual participants vary from each other -- a question that should be addressable even in small samples given the right statistical tools. We propose Neural Topographic Factor Analysis (NTFA), a probabilistic factor analysis model that infers embeddings for participants and stimuli. These embeddings allow us to reason about differences between participants and stimuli as signal rather than noise. We evaluate NTFA on data from an in-house pilot experiment, as well as two publicly available datasets. We demonstrate that inferring representations for participants and stimuli improves predictive generalization to unseen data when compared to previous topographic methods. We also demonstrate that the inferred latent factor representations are useful for downstream tasks such as multivoxel pattern analysis and functional connectivity.

==> algorithmic.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State{} \algorithmicassert(#1)}

\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicdefault{\textbf{default}}
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}
\algdef{SE}[DEFAULT]{Default}{EndDefault}[1]{\algorithmicdefault\ #1}{\algorithmicend\ \algorithmicdefault}
\algtext*{EndSwitch}
\algtext*{EndCase}
\algtext*{EndDefault}

\algnewcommand\algorithmicmatch{\textbf{match}}
\algdef{SE}[MATCH]{Match}{EndMatch}[1]{\algorithmicmatch\ #1}{\algorithmicend\ \algorithmicmatch}
\algtext*{EndMatch}

\algnewcommand\algorithmictry{\textbf{try}}
\algnewcommand\algorithmiccatch{\textbf{catch}}
\algblockdefx[Try]{Try}{EndTry}{\algorithmictry}{\algorithmicend\ \algorithmictry}
\algtext*{EndTry}
\algcblockdefx[Catch]{Try}{Catch}{EndTry}[1]{\algorithmiccatch\ #1}{\algorithmicend\ \algorithmictry}%
\algtext*{EndTry}
\MakeRobust{\Call}

\algdef{SE}[QUERY]{Query}{EndQuery}%
   [2]{\textbf{query}\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\algorithmicend\ \algorithmicquery}%
\algtext*{EndQuery}

\def\@algocf@capt@ruled{under}

